Dissecting the End-to-end Latency of Interactive Mobile Video Applications

In this paper we measure the step-wise latency in the pipeline of three kinds of interactive mobile video applications that are rapidly gaining popularity, namely Remote Graphics Rendering (RGR) of which we focus on mobile cloud gaming, Mobile Augmented Reality (MAR), and Mobile Virtual Reality (MVR). The applications differ from each other by the way in which the user interacts with the application, i.e., video I/O and user controls, but they all share in common the fact that their user experience is highly sensitive to end-to-end latency. Long latency between a user control event and display update renders the application unusable. Hence, understanding the nature and origins of latency of these applications is of paramount importance. We show through extensive measurements that control input and display buffering have a substantial effect on the overall delay. Our results shed light on the latency bottlenecks and the maturity of technology for seamless user experience with these applications.

==> mcglatencypaper-background.tex <==
%Mobile cloud computing has enabled the possibility to offload computation and storage from the resource-limited mobile client to the cloud. %Traditional video services such as YouTube and Netflix are among the most popular cloud services on mobile clients. 
%The evolution of high-speed mobile networks and mobile devices has enabled a new class of interactive, latency-sensitive video applications, such as cloud gaming, augmented reality (AR) and virtual reality (VR) applications. These applications routinely leverage the cloud's computing power to process video and render graphics.

%Recent advances in mobile networks and cloud computing have enabled a new class of interactive, latency-sensitive video applications. In addition to sufficient amount of available bandwidth, low latency is the most critical requirement for the user experience of these applications. % Many of them also require high bandwidth which strains the network even more.

% While deep understanding of the impact of latency on user experience is still an open problem, previous research has discovered many things about human perception of latency with modern mobile technology. For example, Deber et al. recently characterized the Just Noticeable Difference (JND) and the impact of additional latency on task performance in direct and indirect user interaction with a touch device\cite{deber2015much}. They found that the mean JND for a simple tapping task is 69 ms and 96 ms for direct and indirect touch, respectively. The JND is substantially shorter when performing a dragging task. Lee et al. studied error rates in pointing tasks where a target is about to appear within a limited time window for selection\cite{lee2016chi}.% , which is highly relevant in our target applications. 
% They found out that variability in the timing of the pointing event results in lower than expected performance. %Therefore, it is important to also understand the variation in the different latency components.
% Janzen et al. confirmed in their studies that high latency and low frame rate have a negative impact on user performance in selecting moving targets \cite{janzen2014chi}.
 
% The quest for low latency with mobile applications has mostly focused on making the network delay shorter through novel architectures. For example, Satyanarayanan et al. have presented Cloudlets that offer computing power for mobile clients within one-hop latency\cite{satyanarayanan2009case}. Clinch et al. investigated the impact of Cloudlet proximity on user experience with a simple game\cite{clinch2012percom}. Their results also confirm that closeness improves user experience but they could not precisely quantify how close is close enough. A more incremental approach by Choy et al. is to use the existing CDN network to offload computation from the mobile device\cite{choy2014hybrid}. Network latency together with access delay is however only part of the delay pipeline in latency-critical mobile video applications. Processing delay on the server side as well as on the client side occur both in the software and hardware. In this paper we mainly focus on the client side latency.% build-up using real use cases of delay-sensitive video applications.

% Within the class of RGR applications, cloud gaming has received relatively much attention from the research community.
% Jarschel et al. have shown that the cloud gaming experience is highly sensitive to delay\cite{jarschel2011evaluation}. Most studies have concentrated on simulating the varying delay under different network conditions. However, recent results from Raaen et al. show that gaming setups can have significant base delays even in optimal conditions\cite{raaen2014can}. Lee et al. proposed to speculatively execute different possible scenarios of a cloud game in order to mask latency\cite{lee2015mobisys}. In this paper we further dissect the different delay components affecting the total delay experienced by the user particularly in a mobile cloud gaming application. 

%We are currently witnessing the rise of augmented (AR) and virtual (VR) reality applications. %Such applications use the motion sensors of the mobile phone to track the orientation of the device and use the information to render either added objects to a projection of the real world captured with the device's camera (AR) or complete virtual worlds (VR). 
%, we analyze the latencies involved in the core steps of a typical AR application.
%In VR measurements we use the latest Daydream compatible hardware to get up-to-date information on the latencies involved in today's mobile phone powered VR applications.

%The delay components of delay-sensitive video applications such as a cloud gaming client have been 

Concerning measurement methods, previous studies have mostly used either timing hooks injected directly into the code or a high-speed camera\cite{chen2014TMM,ivkovic2015chi,chang2016mm}. A predictive approach has also been proposed by Cattan et al. but it requires separate calibration\cite{cattan2015its}. Timing hooks are useful for measuring independent tasks occurring completely in the mobile device, whereas a high-speed camera can only capture the total delay from a control press to display update. A more detailed break down of delay components requires new novel methods. In this paper we utilize a modified and extended version of the WALT Latency Timer \cite{google_walt} together with code injections to further dissect the delay pipeline. Similar measurement setups have been previously utilized successfully in measuring mobile phone display responsiveness \cite{beyer2015method,deber2016hammer}. In addition to these setups, our approach can also measure gyro, gamepad and Bluetooth delay on top of the traditional touch latency measurements. Our setup is also in-sync with the mobile phone, allowing a more precise division of latency components.


